Neural Execution Engines: Learning to Execute Subroutines

A significant effort has been made to train neural networks that replicate algorithmic reasoning, but they often fail to learn the abstract concepts underlying these algorithms. This is evidenced by their inability to generalize to data distributions that are outside of their restricted training sets, namely larger inputs and unseen data. We study these generalization issues at the level of numerical subroutines that comprise common algorithms like sorting, shortest paths, and minimum spanning trees. First, we observe that transformer-based sequence-to-sequence models can learn subroutines like sorting a list of numbers, but their performance rapidly degrades as the length of lists grows beyond those found in the training set. We demonstrate that this is due to attention weights that lose fidelity with longer sequences, particularly when the input numbers are numerically similar. To address the issue, we propose a learned conditional masking mechanism, which enables the model to strongly generalize far outside of its training range with near-perfect accuracy on a variety of algorithms. Second, to generalize to unseen data, we show that encoding numbers with a binary representation leads to embeddings with rich structure once trained on downstream tasks like addition or multiplication. This allows the embedding to handle missing data by faithfully interpolating numbers not seen during training.

==> sections/failure.tex <==
\vspace{-.3cm}
\section{Current Limitations of Sequence to Sequence Generalization}
\label{section:sorting}
\vspace{-.3cm}

% \subsection{Learning Selection Sort}
% \label{section:s2ssort}
% \vspace{-.3cm}
%In this section, we demonstrate that state-of-the-art sequence to sequence models fail to generalize to longer sequences, and provide explanations by examining its attention weights.
% \reminder{let's add an opening to this section so that the reader knows what to expect here}

\paragraph{Learning Selection Sort}
We first study how well a state-of-the-art transformer-based sequence to sequence model (Section \ref{section:transformers}) learns selection sort. Selection sort involves iteratively finding the minimum number in a list, removing that number from the list, and adding it to the end of the sorted list. We model selection sort using sequence to sequence learning~\cite{sutskever2014sequence} with input examples of unsorted sequences (length $\leq$ $L$) of $n$-bit binary numbers ($L$=8 and $n$=8) and output examples of the correctly sorted sequence. To imitate a sorting subroutine, we provide supervision on intermediate states: at each stage of the algorithm the transformer receives the unsorted input list, the partially sorted output list, and the target number.
% The current state of the algorithm is therefore specified by the full input sequence and the current partial output sequence.

\begin{figure}
\vspace{-0.5cm}
    \centering
    \begin{minipage}{.45\textwidth}
        \includegraphics[width=\textwidth]{Figs/failure_annotated_3_lines_old.pdf}
        \caption{Sorting performance of transformers trained on sequences of up to length 8.}
        \vspace{-0.1cm}
        \label{fig:s2sperformance}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
    \includegraphics[width=\textwidth]{Figs/fuzzy-clear-attn-v2.pdf}
        \caption{Visualizing decoder attention weights. Attention is over each row. Transformer attention saturates as the output sequence length increases, while NEE maintains sharp attention.}
        \label{fig:ssattention}
    \end{minipage}
\vspace{-0.5cm}
\end{figure}
\vspace{-0.2cm}
The numbers used as inputs and outputs to a vanilla transformer are one-hot encoded. Later, we will explore performance when the numbers are binary encoded (Section~\ref{sec:number-representations})\footnote{We also experimented with one-hot 256-dimensional outputs for other approaches used in the paper with similar results. See the supplementary material.}. The decoder uses a greedy decoding strategy.

% The inputs to the encoder and decoder \yy{of a vanilla transformer are sequences of one-hot} embedded vectors while those of a modified transformer and NEE are sequences of bitwise embedded vectors (Section~\ref{sec:number-representations}). The decoder uses a greedy decoding strategy.
% The outputs of the decoder are one-hot $256$-dimensional vectors representing the unnormalized log-probabilities of the output numbers.
% The outputs of the decoder \yy{of a vanilla transformer are one-hot vectors in contrast to 8-bit binary vectors for modified transformer and NEE.} 

We find that uniformly random numbers are easier to sort than distributions with more similar numbers (e.g., 1 vs. 2, 53 vs. 54). We therefore include both kinds of distributions in the training set\footnote{Throughout this work, the preponderance of errors are regenerated numbers that are off by small differences.}  (95\% random numbers, 5\% numbers with small differences).


% \begin{wrapfigure}{r}{8cm}
%   \vspace{-.5cm}
%   \centering
%   \includegraphics[width=.52\textwidth]{Figs/fuzzy-clear-attn-v2.pdf}
%   \vspace{-0.2cm}
%   \caption{Visualizing decoder attention weights. Attention is over each row. Transformer attention saturates as the output sequence length increases, while NEE maintains sharp attention.}
%   \label{fig:ssattention}
%   \vspace{-0.5cm}
% \end{wrapfigure}

The performance of this vanilla transformer, evaluated as achieving an exact content and positional match to the correct output example, is shown in Figure \ref{fig:s2sperformance} (where the test distribution consists of 60\% random numbers and 40\% numbers with small differences). The transformer is able to learn to sort the test-length distribution (at 8 numbers), but performance rapidly degrades as the input data distribution shifts to longer sequences and by 100 integers, performance is under 10\%.
%%%%%%%%%%%%% failure_annotated_3_lines.pdf to change to 3 lines

One of the main issues we found is that the transformer has difficulty distinguishing close numbers. We make a number of small architectural modifications in order to boost its accuracy. We describe these modifications, and provide ablations in Appendix~\ref{app:ablation}. 
% In an attempt to increase performance, we make a number of modifications to better tune the encoder to process binary numbers. These modifications are driven by the unsatisfactory performance of the vanilla transformer in distinguishing close numbers (Appendix~\ref{app:ablation}, Figure \ref{fig:appendix_granularity_wo_feedback}). To aid in the ability of the number to learn numerical similarity in carry-out cases when many bits flip (32 vs. 31, 64 vs. 63), we use bitwise embeddings and replace the dot product self-attention with a symmetric feed-forward self-attention (Figure \ref{fig:appendix_granularity_wo_feedback}). To help handle small differences in general, we use shared instead of independent linear projections of queries, keys and values. To aid in reconstructing small numerical differences, we scale up the residual connection strength by a factor of $1.5$. We provide an ablation study of these modifications in the supplementary material.
% These modifications over the original transformer model are shown in the Appendix (Figure~\ref{fig:transformer-modified}). 
%
As Figure~\ref{fig:s2sperformance} shows, given these modifications, sequence-to-sequence transformers are capable of learning this algorithm on sequences of length $\leq 8$ with a high degree of accuracy, reaching almost perfect accuracy with proper modifications. However, the model fails to generalize to longer sequences than those seen at training time, and performance also sharply drops as the sequence length increases.
% Figure~\ref{fig:s2sperformance} shows the sorting performance of five models: (1) the model with all the modifications mentioned above, (2) the model with all modifications but with non-symmetric attention, (3) the model with all modifications but with dot-product attention (instead of symmetric feed-forward self-attention), (4) the vanilla transformer model with bitwise embedding, and (5) the vanilla transformer model with one-hot embedding (which is default in NLP). The results of more variants and data mixes are shown in the Appendix.   




% \vspace{-.3cm}  
% \subsection{Attention Fidelity}
% \label{subsec:s2ssort}
% \vspace{-.3cm}

\paragraph{Attention Fidelity}
To understand why performance degrades as the test sequences get longer, we plot the attention matrix of the last layer in the decoder (Figure \ref{fig:ssattention}a). During decoding, the transformer accurately attends to the first few numbers in the sequence (distinct dots in the chart) but the attention distribution becomes ``fuzzy'' as the number of decoding steps increases beyond 8 numbers, often resulting in the same number being repeatedly predicted. 

Since the transformer had difficulty clearly attending to values beyond the training sequence length, we separate the supervision of \emph{where} the computation needs to occur from \emph{what} the computation is. \emph{Where} the computation needs to occur is governed by the transformer mask. To avoid overly soft attention scores, we aim to restrict the locations in the unsorted sequence where the transformer could possibly attend in every iteration. This is accomplished by producing a conditional mask which learns to ignore the data elements that have already been appended to the \texttt{sorted\_list} and feed that mask back into the transformer (shown on the bottom-left side of Figure \ref{fig:algorithms}). Put another way, we have encoded the current algorithmic state (the sorted vs. unsorted list elements) in the attention mask rather than the current decoder output.

This modification separates the control (which elements should be considered) from the computation itself (find the minimum value of the list). This allows the transformer to learn output logits of much larger magnitude, resulting in sharper attention, as shown in Figure~\ref{fig:ssattention}b. Our experimental results consequently demonstrate strong generalization, sorting sequences of up to length 100 without error, as shown in Figure~\ref{fig:s2sperformance}. Next, we evaluate this mechanism on a variety of other algorithms.
